Improving Chemical Understanding of LLMs via SMILES Parsing

Large language models (LLMs) are increasingly recognized as powerful tools for scientific discovery, particularly in molecular science. A fundamental requirement for these models is the ability to accurately understand molecular structures, commonly encoded in the SMILES representation. However, current LLMs struggle to interpret SMILES, even failing to carry out basic tasks such as counting molecular rings. To address this limitation, we introduce CLEANMOL, a novel framework that formulates SMILES parsing into a suite of clean and deterministic tasks explicitly designed to promote graph-level molecular comprehension. These tasks span from subgraph matching to global graph matching, providing structured supervision aligned with molecular structural properties. We construct a molecular pretraining dataset with adaptive difficulty scoring and pre-train open-source LLMs on these tasks. Our results show that CLEANMOL not only enhances structural comprehension but also achieves the best or competes with the baseline on the Mol-Instructions benchmark.

==> 2.motivation_pretrain.tex <==
\section{Motivation (v2): Unclear pretraining tasks in molecular domains}

Pretraining tasks should be intuitive, well-structured, and sufficiently easy to guide the model toward generalization. The intuition can be drawn from human learning: before students are asked to solve complex mathematical problems, they must first master basic concepts such as numbers and arithmetic. The curriculum is structured to reflect increasing difficulty, grounded in deterministic, well-defined exercises. This principle also applies to large language models (LLMs), whose general capabilities are often strengthened through pretraining on structured tasks with well-defined solutions, such as program synthesis or mathematical problem solving \citep{guo2023can, XX, XX}.


In the molecular domain, however, the design of pretraining tasks remains largely underexplored and often lacks clarity. Most prior works adopt task formulations from natural language processing, such as masked language modeling (MLM) \citep{devlin2019bert} or sequence-to-sequence translation \citep{raffel2020t5}, applying them to molecular string representations like SMILES \citep{weininger1988smiles} or SELFIES \citep{krenn2020self} and their textual descriptions \citep{pei-etal-2023-biot5, edwards2022molt5}. These approaches introduce ambiguity in the supervision signal due to the inherent non-determinism.

% figure that describes masking of F -> O could be another answer
\input{figure/fig_2_problem_pretrain}

In detail, as illustrated in \cref{fig:2_problem_pretrain}, masked SMILES prediction suffers from ambiguous supervision: multiple chemically valid tokens may occupy the same masked position (e.g., substituting different atoms from the same group). This creates uncertainty during training, where the model is penalized for generating chemically correct, yet mismatched, answers. Such ambiguity makes it difficult for the model to possess appropriate molecular understanding.

-------

To address this issue, we propose a novel pretraining framework grounded in SMILES parsing, a task that is both structurally simple and deterministically solvable. SMILES parsing is to infer molecular structure from SMILES strings through deterministic tasks such as counting atoms and bonds, identifying subgraphs, and canonicalizing representations. These tasks provide unambiguous supervision, enabling models to acquire foundational chemical knowledge without the noise of ambiguous labels.

\paragraph{SMILES parsing task description.} We define SMILES parsing as a suite of three deterministic task categories: enumeration, subgraph matching, and traversal, as described in \cref{fig:2_smiles_parsing}. Each category is designed to reflect a specific aspect of molecular structure interpretation, with clearly defined solutions.

\input{figure/fig_2_smiles_parsing}

\begin{itemize}
    \item \textbf{Enumeration.} This category includes \textit{atom counting} and \textit{bond counting}, where the model predicts the number of atoms or bonds of a specific type within the molecule. These tasks teach basic structural information, enabling the model to capture atomic composition and bonding patterns within a molecule.
    
    \item \textbf{Subgraph Matching.} This includes \textit{ring counting} and \textit{chain length measurement}. Ring counting involves identifying the number of rings of a particular size (e.g., five- or six-membered rings), while chain length measurement targets the length of the longest carbon chain excluding rings. These tasks enhance the recognition of common molecular motifs and branching patterns.

    \item \textbf{Traversal.} The traversal task focuses on \textit{SMILES canonicalization}, where the model converts randomly ordered SMILES into their canonical form. Since SMILES representations are non-unique due to atom ordering and branching, this task trains the model to uncover the underlying molecular graph structure regardless of permutation.
\end{itemize}

\input{figure/fig_2_edge_case}
% TODO: bar plot of 5-shot in table 1
\input{figure/fig_2_failure}

\paragraph{Failure of recent LLMs.} Although SMILES parsing may appear to be a straightforward task—requiring only basic structural understanding—it poses surprising challenges for current large language models (LLMs). In particular, edge cases involving complex branching or multiple ring structures can make seemingly simple questions difficult to resolve accurately. As shown in \cref{fig:2_edge_case}, the grammar complexity of such SMILES strings can obscure the understanding of underlying molecular graphs, making it challenging for the model to accurately track the required molecular structural information.

We observe that even state-of-the-art general-purpose LLMs, including GPT-4o \citep{openai2024gpt4technicalreport} and DeepSeek-V3-Chat \citep{liu2024deepseek}, struggle with SMILES parsing, achieving no more than 60\% accuracy across representative tasks, as described in \cref{fig:2_failure}. This failure is notable given these models’ strong performance in other structured domains such as mathematics and code generation. The inability of these models to handle even basic molecular parsing tasks underscores a critical gap in their structural understanding and motivates the need for explicit pretraining strategies tailored to molecules.



==> figure/fig_2_smiles_parsing_task.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/fig_2_smiles_parsing_task_.pdf}
    \caption{\textbf{Illustration of SMILES parsing tasks.} Each column visualizes one of the five SMILES parsing tasks: (1) functional group matching, (2) ring counting, (3) carbon chain length measurement, (4) SMILES canonicalization, and (5) fragment assembly. The highlighted tokens in the SMILES strings correspond to the molecular substructures involved in each task.}
    \label{fig:2_smiles_parsing_task}
\end{figure}

==> figure_appx/fig_appx_1_parsing_prompt.tex <==
\begin{figure*}
  \centering
  \resizebox{0.9\linewidth}{!}{
  \begin{tcolorbox}[
    colback=gray!5!white, 
    colframe=gray!60!black,
    title={
      \parbox[t]{\dimexpr\linewidth-4mm\relax}{%
        \ttfamily
        SMILES: c1ccc(C(F)(F)F)c(N2C(N)=C(C\#N)[C@H](c3cc(OCC)ccc3OCC)C3=C2CCCC3=O)c1
        

      }
    }
  ]
  \begin{tabularx}{\textwidth}{>{\bfseries}lX}
  \multicolumn{2}{l}{\textcolor{gray}{\# Functional group}} \\
    Question:& Given the SMILES, determine inclusion of the functional group COC.  \\
    Answer:& Yes \\
    \multicolumn{2}{l}{\textcolor{gray}{\# Ring}} \\
    Question:& Calculate the count of SIX-membered rings in the given SMILES string. \\
    Answer: & 4 \\
    % \\
    \multicolumn{2}{l}{\textcolor{gray}{\# Canonicalization}} \\
    Question: & Give me a canonicalized SMILES that represents the same given molecule.\\
    Answer:  & CCOc1ccc(OCC)c([C@H]2C(C\#N)=C(N)N(c3ccccc3C(F)F)F)C3=C2C(=O)CCC3)c1 
    \\
    
    
  \end{tabularx}
  \end{tcolorbox}
  }
    \caption{\textbf{Examples of few-shot prompts for SMILES parsing.} }\label{fig:2_smiles_parsing}
    % }
\end{figure*}

==> table/tab_2_pattern_memorization.tex <==
\begin{table}
    \centering
    \caption{\textbf{Results of failure of LLMs with pattern memorization.} Ratio indicates the proportion of consistent model predictions across different SMILES permutations of the same molecule.
}
    \label{tab:2_pattern_memorization}
    \begin{tabular}{cc}
    \toprule[1.25pt]
    Task & Ratio \\
    \midrule[1.25pt]
     Retrosynthesis    &  \\
     Forward reaction prediction    & 0.123 \\ 
     \bottomrule[1.25pt]
    \end{tabular}
    
\end{table}

==> table/tab_5_ablation.tex <==
\begin{table}
    \centering
    \caption{\textbf{Ablation study on pattern memorization.} Ratio indicates the proportion of consistent model predictions across different SMILES permutations of the same molecule.
}
    \label{tab:5_ablation}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}
    \toprule[1.25pt]
    Task & Retro. & Forward. & Reagent.  \\
    \midrule[1.25pt]
     Mol-Instructions (SFT)    & & 0.123 & \\ 
     \Algname (Ours) & & 0.154 & \\
     \bottomrule[1.25pt]
    \end{tabular}
    }
    
\end{table}
